Motivated Reasoning and the Political Economy of Climate Change Inaction

We study how motivated reasoning affects the provision of climate policy in an electoral competition framework. Voters experience anticipatory disutility when future outcomes appear grim and may therefore distort beliefs in response to adverse information. We develop a game-theoretic model in which voters and politicians receive signals about the severity of climate change. When the anticipated welfare losses from severe climate change are sufficiently large, voters optimally ignore unfavorable information, inducing politicians to campaign on policies appropriate for mild climate change only. When welfare losses are moderate, the model admits a second, efficient equilibrium in which voters trust politicians to implement welfare-maximizing policies and vote informatively, thereby creating incentives for politicians to propose adequate climate policy. The model shows how motivated belief formation and voters' expectations about policy responsiveness jointly determine equilibrium selection between effective climate policy and persistent political inaction.

==> todo.tex <==
Journal Lis:

-JPUBE
-EJ
-JEEM
-QJPS
-JEBO


What to do
-rerun regression with GDP PC instead of CC Risk
-mention LOO in main text as robustness


